Improved replica bounds for the independence ratio of random regular graphs

Studying independent sets of maximum size is equivalent to considering the hard-core model with the fugacity parameter $\lambda$ tending to infinity. Finding the independence ratio of random $d$-regular graphs for some fixed degree $d$ has received much attention both in random graph theory and in statistical physics. For $d \geq 20$ the problem is conjectured to exhibit 1-step replica symmetry breaking (1-RSB). The corresponding 1-RSB formula for the independence ratio was confirmed for (very) large $d$ in a breakthrough paper by Ding, Sly, and Sun. Furthermore, the so-called interpolation method shows that this 1-RSB formula is an upper bound for each $d \geq 3$. For $d \leq 19$ this bound is not tight and full-RSB is expected. In this work we use numerical optimization to find good substituting parameters for discrete $r$-RSB formulas ($r=2,3,4,5$) to obtain improved rigorous upper bounds for the independence ratio for each degree $3 \leq d \leq 19$. As $r$ grows, these formulas get increasingly complicated and it becomes challenging to compute their numerical values efficiently. Also, the functions to minimize have a large number of local minima, making global optimization a difficult task.

==> declarations.tex <==
\section*{Declarations}

\subsection*{Funding}
This work was supported by the MTA-R\'enyi Counting in Sparse Graphs ``Momentum'' Research Group and NRDI 
%(National Research, Development and Innovation Office) 
grant KKP 138270.

\subsection*{Conflicts of interest/Competing interests} 
The author declares that he has no conflict of interest.

\subsection*{Availability of data}
The datasets needed to recover the claimed bounds of the current paper are available in a Github repository:\\ \url{https://github.com/harangi/rsb/blob/5f2ea09166a1931c3bae5e05afaee13093015b53/examples.sobj}


